The Bispectrum in the Effective Field Theory of Large Scale Structure

We study the bispectrum in the Effective Field Theory of Large Scale Structure, consistently accounting for the effects of short-scale dynamics. We begin by proving that, as long as the theory is perturbative, it can be formulated to arbitrary order using only operators that are local in time. We then derive all the new operators required to cancel the UV-divergences and obtain a physically meaningful prediction for the one-loop bispectrum. In addition to new, subleading stochastic noises and the viscosity term needed for the one-loop power spectrum, we find three new effective operators. The three new parameters can be constrained by comparing with N-body simulations. The best fit is precisely what is suggested by the structure of UV-divergences, hence justifying a formula for the EFTofLSS bispectrum whose only fitting parameter is already fixed by the power spectrum. This result predicts the bispectrum of N-body simulations up to $k \approx 0.22\, h\, \text{Mpc}^{-1}$ at $z=0$, an improvement by nearly a factor of two as compared to one-loop standard perturbation theory.

==> fitparams_resc.tex <==
3 parameters & --- & $11.22\pm 5.31$ & $101.05\pm 27.26$ & $60.59\pm 26.19$ & $48.23\pm0.96$ & $1$\\ 
4 parameters & --- & $-14.60\pm 131.39$ & $88.86\pm 67.71$ & $48.35\pm 67.53$ & $57.14\pm 45.30$ & $1$\\ 
\hline 
3 parameters & --- & $8.82\pm 7.28$ & $136.27\pm 37.35$ & $72.32\pm 35.89$ & $73.84\pm1.48$& $5/3$\\ 
4 parameters & --- & $-27.78\pm 186.21$ & $119.16\pm 94.69$ & $53.56\pm 101.90$ & $87.47\pm 69.34$ & $5/3$\\ 
